Fast Trajectory Optimization for Legged Robots using Vertex-based ZMP Constraints

This paper combines the fast Zero-Moment-Point (ZMP) approaches that work well in practice with the broader range of capabilities of a Trajectory Optimization formulation, by optimizing over body motion, footholds and Center of Pressure simultaneously. We introduce a vertex-based representation of the support-area constraint, which can treat arbitrarily oriented point-, line-, and area-contacts uniformly. This generalization allows us to create motions such quadrupedal walking, trotting, bounding, pacing, combinations and transitions between these, limping, bipedal walking and push-recovery all with the same approach. This formulation constitutes a minimal representation of the physical laws (unilateral contact forces) and kinematic restrictions (range of motion) in legged locomotion, which allows us to generate various motion in less than a second. We demonstrate the feasibility of the generated motions on a real quadruped robot.

==> tex/com_collocation_part.tex <==
% direct collocation approaech
\subsubsection{Collocation}
Another approach is to represent the \gls{com} motion by segments of cubic polynomials
and optimize over the \gls{com} position and velocity at the intersections, so
\begin{align}
\state(t) 
&= 
\begin{bmatrix}
\cxy(t) \\
\cxyd(t)
\end{bmatrix}
=
\sum_{\idxorder=0}^3
\begin{bmatrix}
\poly_{\idxpoly,\idxorder} \\
\polyv_{\idxpoly,\idxorder}
\end{bmatrix}
\tlocal^\idxorder,
\\
\comdecision &= 
\begin{bmatrix}
\cxy_1,\cxyd_1,\dots,\cxy_\numpoly,\cxyd_\numpoly
\end{bmatrix}.
\label{eq:com_poly_col}
\end{align}
When parameterizing the polynomial to comply with the system dynamics \eref{eq:lip_ode}
at the start and end of each segment, the polynomial 
coefficients $\poly_{\idxpoly,\idxorder}, \polyv_{\idxpoly,\idxorder} \in \real{2}$ can be fully represented
by the position $\cxy_\idxpoly$, velocity
$\cxyd_\idxpoly$ and the \gls{cop} $\uxy_{\idxnode}$ at the neighboring nodes ${\idxnode}$ and ${\idxnode+1}$
(see \aref{ap:dynamic_constraint}).
%
Again, this will only comply with the system dynamics at the nodes $\idxpoly$,
but there is no guarantee that the input $\uxy_\idxnode$ will drive the system to the next state. 
By enforcing the system dynamics at the center $t_c$ between nodes, we are implicitly
enforcing a Simpson Integration Rule
by the constraint
\begin{equation}
\stated[t\!=\!t_c] =
\sum_{\idxorder=1}^3 \idxorder 
\begin{bmatrix}
\poly_{\idxpoly,\idxorder} \\
\polyv_{\idxpoly,\idxorder}
\end{bmatrix}
\tlocal^{\idxorder-1}
=
\func(\state[t], \frac{\uxy_\idxnode+\uxy_{\idxnode+1}}{2}).
\end{equation}
This way of enforcing the continous system dynamics in a discrete setting is called
``collocation'' \cite{Hargraves1987}.




% this part was in appendix
\subsubsection{Position/Velocity Polynomial Formulation}
In this formulation known as ``collocation'', the position and velocity is represent as two separate
cubic polynomials
\begin{equation*}
\state(t) 
= 
\begin{bmatrix}
\cxy(t) \\
\cxyd(t)
\end{bmatrix}
=
\sum_{\idxorder=0}^3 
\begin{bmatrix}
\poly_{\idxpoly,\idxorder} \\
\polyv_{\idxpoly,\idxorder}
\end{bmatrix}
(t-t_\idxnode)^\idxorder
\end{equation*}
Enforcing the system dynamics at the nodes, the coefficients 
$\poly_{\idxpoly,\idxorder}, \polyv_{\idxpoly,\idxorder} \in \real{2}$ 
can be fully represented by the state derivative at the neighboring
nodes \cite{VonStryk1992} as
%
\begin{align*}
\begin{bmatrix} \poly_{k,0}^T & \polyv_{k,0}^T \end{bmatrix}^T &= \state_\idxnode \\
\begin{bmatrix} \poly_{k,1}^T & \polyv_{k,1}^T \end{bmatrix}^T &= \func_\idxnode \\
\begin{bmatrix} \poly_{k,2}^T & \polyv_{k,2}^T \end{bmatrix}^T &= \dt^{-2} (3\state_\idxnode - 2\dt \func_\idxnode + 3\state_{\idxnode+1} - \dt \func_{\idxnode+1}) \\
\begin{bmatrix} \poly_{k,3}^T & \polyv_{k,3}^T \end{bmatrix}^T &= \dt^{-3} (2\state_\idxnode + \dt \func_\idxnode - \state_{\idxnode+1} + \dt \func_{\idxnode+1})
\end{align*}
where
$
\func_\idxnode =
\func(\state_\idxnode, \control_\idxnode)
%=
%\begin{bmatrix}
%\cxyd_\idxnode \\
%\frac{g}{h}(\cxy_\idxnode - \uxy_\idxnode)
%\end{bmatrix}
$
represents the derivative of second-order system dynamics evaluated at time $t_\idxnode$,
and $\dt = t_{\idxnode+1} - t_\idxnode$ represents the duration of each polynomial.



